IoT-AD: A Framework To Detect Anomalies Among Interconnected IoT Devices

In an Internet of Things (IoT) environment (e.g., smart home), several IoT devices may be available that are interconnected with each other. In such interconnected environments, a faulty or compromised IoT device could impact the operation of other IoT devices. In other words, anomalous behavior exhibited by an IoT device could propagate to other devices in an IoT environment. In this paper, we argue that mitigating the propagation of the anomalous behavior exhibited by a device to other devices is equally important to detecting this behavior in the first place. In line with this observation, we present a framework, called IoT Anomaly Detector (IoT-AD), that can not only detect the anomalous behavior of IoT devices, but also limit and recover from anomalous behavior that might have affected other devices. We implemented a prototype of IoT-AD, which we evaluated based on open-source IoT device datasets as well as through real-world deployment on a small-scale IoT testbed we have built. We have further evaluated IoT-AD in comparison to prior relevant approaches. Our evaluation results show that IoT-AD can identify anomalous behavior of IoT devices in less than 2.12 milliseconds and with up to 98% of accuracy.

==> sections/Motivation.tex <==
\section{Use Cases and Motivation}
\label{sec:overview}

\textbf{Scenario 1:}
Lets assume the thermostat of the smart home got compromised. The thermostat triggered on the heater instead of AC, that can lead the temperature 90 Fahrenheit or more. In addition to these, the thermostat interacted with smart humidifier and turned it off. This situation can create health hazard for the resident and if it keeps longer in that state then the heater can cause fire incident.
Similarly, because of the false reading of thermostat, AC can be triggered on instead of the heater. Also, smart thermostat interacted with smart blinds to turn it off. This situation can lead the room colder and cause problematic environment for people who have breathing problems.

\textbf{Scenario 2:}
A smart fish tank that is created with multiple IoT devices (\eg Smart water quality sensor, smart fish feeder, smart temperature controller, smart water changer, Oxygen diffuser, etc.). False reading of smart water quality sensor can triggered on the oxygen diffuser, water changer, and the smart fish feeder. Excessive oxygen, fish food or other chemical ingredient can lead the fishes to die.

\textbf{Scenario 3:}

%child bedroom-> motion sensor-> light turned on-> baby monitor-> 
laundry room->For example, in the laundry room if the washer is turned on it will turn on the fan to keep the room cool and also it will turn on the dehumidifier to keep the room humid in balance. As a result when the controller detects the wrong value of dehumidifier it will use the interaction tree to find out the source and the affected device. In this scenario, the value of washers’ state was falsely sent to the controller that started propagating a malicious event and turned on the fan and the dehumidifier. 

